Demonstrating Data-to-Knowledge Pipelines for Connecting Production Sites in the World Wide Lab

The digital transformation of production requires new methods of data integration and storage, as well as decision making and support systems that work vertically and horizontally throughout the development, production, and use cycle. In this paper, we propose Data-to-Knowledge (and Knowledge-to-Data) pipelines for production as a universal concept building on a network of Digital Shadows (a concept augmenting Digital Twins). We show a proof of concept that builds on and bridges existing infrastructure to 1) capture and semantically annotates trajectory data from multiple similar but independent robots in different organisations and use cases in a data lakehouse and 2) an independent process that dynamically queries matching data for training an inverse dynamic foundation model for robotic control. The article discusses the challenges and benefits of this approach and how Data-to-Knowledge pipelines contribute efficiency gains and industrial scalability in a World Wide Lab as a research outlook.

==> 99_Notes.tex <==
•	Timeline: Preprint 01.08.24
•	Publication Process:
o	Preprint
o	CAIsE: journal first session (i.e. we still have to decide on a journal)
 
Writing Style is not hierarchical, i.e. constructive criticism is welcome. Or please change minor things directly.
Open points that we should discuss: Definition Data to Knowledge Pipeline.
 
@all: Please send around papers you now that address digital shadows from the cluster perspective.
@Philipp: Please ask Judith for her “best digital shadow” paper
@Leon: Get in touch with David on further data generation
 
Keep a larger vision of the data-to-knowledge in mind: Multiple companies, multiple domains, autonomous decision.

